Accelerating Algebraic Multigrid Methods via Artificial Neural Networks

We present a novel deep learning-based algorithm to accelerate - through the use of Artificial Neural Networks (ANNs) - the convergence of Algebraic Multigrid (AMG) methods for the iterative solution of the linear systems of equations stemming from finite element discretizations of Partial Differential Equations (PDE). We show that ANNs can be successfully used to predict the strong connection parameter that enters in the construction of the sequence of increasingly smaller matrix problems standing at the basis of the AMG algorithm, so as to maximize the corresponding convergence factor of the AMG scheme. To demonstrate the practical capabilities of the proposed algorithm, which we call AMG-ANN, we consider the iterative solution of the algebraic system of equations stemming from finite element discretizations of two-dimensional model problems. First, we consider an elliptic equation with a highly heterogeneous diffusion coefficient and then a stationary Stokes problem. We train (off-line) our ANN with a rich dataset and present an in-depth analysis of the effects of tuning the strong threshold parameter on the convergence factor of the resulting AMG iterative scheme.

==> tables/m1r2_120.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.18627450980392157,0.47309355683601007,0.9697969360350095}
\definecolor{ccc1_1}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc1_2}{rgb}{0.37450980392156863,0.19584546700716696,0.9951469164070644}
\definecolor{ccc1_3}{rgb}{0.38235294117647056,0.18374951781657034,0.9957341762950345}
\definecolor{ccc1_4}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc1_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc1_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc1_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_0}{rgb}{0.20980392156862748,0.44021574083098725,0.9741386021045101}
\definecolor{ccc2_1}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_3}{rgb}{0.37450980392156863,0.19584546700716696,0.9951469164070644}
\definecolor{ccc2_4}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_5}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_6}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc2_7}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc3_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc3_1}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc3_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_3}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc3_5}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_6}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc3_7}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc4_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc4_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc4_2}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc4_3}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc4_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc4_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc4_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc4_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc5_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc5_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc5_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_3}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc5_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc5_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc6_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc6_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc6_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_3}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc6_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc7_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc7_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc7_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc7_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc8_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc8_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc8_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc8_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc9_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc9_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc9_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc9_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc10_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc10_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc10_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc10_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc11_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc11_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc11_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc11_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$ & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.091(9) & \cellcolor{ccc1_1!20} 0.069(8) & \cellcolor{ccc1_2!20} 0.058(8) & \cellcolor{ccc1_3!20} 0.057(8) & \cellcolor{ccc1_4!20} 0.060(9) & \cellcolor{ccc1_5!20} 0.061(9) & \cellcolor{ccc1_6!20} 0.062(9) & \cellcolor{ccc1_7!20} 0.066(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.087(9) & \cellcolor{ccc2_1!20} 0.066(8) & \cellcolor{ccc2_2!20} 0.059(8) & \cellcolor{ccc2_3!20} 0.058(8) & \cellcolor{ccc2_4!20} 0.059(9) & \cellcolor{ccc2_5!20} 0.060(9) & \cellcolor{ccc2_6!20} 0.061(9) & \cellcolor{ccc2_7!20} 0.068(10)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.085(9) & \cellcolor{ccc3_1!20} 0.066(8) & \cellcolor{ccc3_2!20} 0.060(8) & \cellcolor{ccc3_3!20} 0.059(8) & \cellcolor{ccc3_4!20} 0.061(9) & \cellcolor{ccc3_5!20} 0.060(9) & \cellcolor{ccc3_6!20} 0.061(9) & \cellcolor{ccc3_7!20} 0.069(10)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.085(9) & \cellcolor{ccc4_1!20} 0.065(8) & \cellcolor{ccc4_2!20} 0.061(8) & \cellcolor{ccc4_3!20} 0.067(9) & \cellcolor{ccc4_4!20} 0.062(9) & \cellcolor{ccc4_5!20} 0.061(9) & \cellcolor{ccc4_6!20} 0.062(9) & \cellcolor{ccc4_7!20} 0.070(10)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.084(9) & \cellcolor{ccc5_1!20} 0.065(8) & \cellcolor{ccc5_2!20} 0.062(8) & \cellcolor{ccc5_3!20} 0.068(9) & \cellcolor{ccc5_4!20} 0.062(9) & \cellcolor{ccc5_5!20} 0.061(9) & \cellcolor{ccc5_6!20} 0.062(9) & \cellcolor{ccc5_7!20} 0.070(10)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.084(9) & \cellcolor{ccc6_1!20} 0.065(8) & \cellcolor{ccc6_2!20} 0.062(8) & \cellcolor{ccc6_3!20} 0.068(9) & \cellcolor{ccc6_4!20} 0.062(9) & \cellcolor{ccc6_5!20} 0.062(9) & \cellcolor{ccc6_6!20} 0.062(9) & \cellcolor{ccc6_7!20} 0.070(10)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.084(9) & \cellcolor{ccc7_1!20} 0.065(8) & \cellcolor{ccc7_2!20} 0.062(8) & \cellcolor{ccc7_3!20} 0.069(9) & \cellcolor{ccc7_4!20} 0.062(9) & \cellcolor{ccc7_5!20} 0.062(9) & \cellcolor{ccc7_6!20} 0.063(9) & \cellcolor{ccc7_7!20} 0.070(10)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.084(9) & \cellcolor{ccc8_1!20} 0.065(8) & \cellcolor{ccc8_2!20} 0.062(8) & \cellcolor{ccc8_3!20} 0.069(9) & \cellcolor{ccc8_4!20} 0.062(9) & \cellcolor{ccc8_5!20} 0.062(9) & \cellcolor{ccc8_6!20} 0.063(9) & \cellcolor{ccc8_7!20} 0.070(10)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.084(9) & \cellcolor{ccc9_1!20} 0.065(8) & \cellcolor{ccc9_2!20} 0.062(8) & \cellcolor{ccc9_3!20} 0.069(9) & \cellcolor{ccc9_4!20} 0.062(9) & \cellcolor{ccc9_5!20} 0.062(9) & \cellcolor{ccc9_6!20} 0.063(9) & \cellcolor{ccc9_7!20} 0.070(10)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.084(9) & \cellcolor{ccc10_1!20} 0.065(8) & \cellcolor{ccc10_2!20} 0.062(8) & \cellcolor{ccc10_3!20} 0.069(9) & \cellcolor{ccc10_4!20} 0.062(9) & \cellcolor{ccc10_5!20} 0.062(9) & \cellcolor{ccc10_6!20} 0.063(9) & \cellcolor{ccc10_7!20} 0.070(10)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.084(9) & \cellcolor{ccc11_1!20} 0.065(8) & \cellcolor{ccc11_2!20} 0.062(8) & \cellcolor{ccc11_3!20} 0.069(9) & \cellcolor{ccc11_4!20} 0.062(9) & \cellcolor{ccc11_5!20} 0.062(9) & \cellcolor{ccc11_6!20} 0.063(9) & \cellcolor{ccc11_7!20} 0.070(10)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.36$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m1r2.tex}}
\end{minipage}

==> tables/m1r2_146.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.18627450980392157,0.47309355683601007,0.9697969360350095}
\definecolor{ccc1_1}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc1_2}{rgb}{0.38235294117647056,0.18374951781657034,0.9957341762950345}
\definecolor{ccc1_3}{rgb}{0.38235294117647056,0.18374951781657034,0.9957341762950345}
\definecolor{ccc1_4}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc1_5}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc1_6}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc1_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc2_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc2_2}{rgb}{0.09215686274509804,0.5977074592660936,0.9491349440359013}
\definecolor{ccc2_3}{rgb}{0.0607843137254902,0.6364742361471413,0.9410892525013715}
\definecolor{ccc2_4}{rgb}{0.009803921568627416,0.7179119230644418,0.9209055179449537}
\definecolor{ccc2_5}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc2_6}{rgb}{0.0725490196078431,0.7829276104921027,0.9005867023006374}
\definecolor{ccc2_7}{rgb}{0.1823529411764706,0.8780812480836979,0.8597998514483725}
\definecolor{ccc3_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc3_1}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc3_2}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc3_3}{rgb}{0.05294117647058827,0.6459280624867872,0.9389883606150565}
\definecolor{ccc3_4}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc3_5}{rgb}{0.025490196078431393,0.7348449670469757,0.9160336012803335}
\definecolor{ccc3_6}{rgb}{0.12745098039215685,0.8336023852211195,0.8810121942857845}
\definecolor{ccc3_7}{rgb}{0.17450980392156867,0.8721195109836108,0.8629289996673897}
\definecolor{ccc4_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc4_1}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc4_2}{rgb}{0.2647058823529412,0.3612416661871529,0.9829730996839018}
\definecolor{ccc4_3}{rgb}{0.04509803921568628,0.6552838500134536,0.9368518385313106}
\definecolor{ccc4_4}{rgb}{0.025490196078431393,0.7348449670469757,0.9160336012803335}
\definecolor{ccc4_5}{rgb}{0.025490196078431393,0.7348449670469757,0.9160336012803335}
\definecolor{ccc4_6}{rgb}{0.11176470588235299,0.8197404829072211,0.8867736859200619}
\definecolor{ccc4_7}{rgb}{0.1588235294117647,0.8597998514483723,0.8690889463055284}
\definecolor{ccc5_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc5_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc5_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc5_3}{rgb}{0.03725490196078429,0.664540178707858,0.9346797673211106}
\definecolor{ccc5_4}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc5_5}{rgb}{0.0490196078431373,0.7594049166547072,0.9084652718195236}
\definecolor{ccc5_6}{rgb}{0.12745098039215685,0.8336023852211195,0.8810121942857845}
\definecolor{ccc5_7}{rgb}{0.17450980392156867,0.8721195109836108,0.8629289996673897}
\definecolor{ccc6_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc6_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc6_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc6_3}{rgb}{0.013725490196078438,0.6916984393193699,0.9279510898565747}
\definecolor{ccc6_4}{rgb}{0.0490196078431373,0.7594049166547072,0.9084652718195236}
\definecolor{ccc6_5}{rgb}{0.056862745098039236,0.767362681448697,0.9058734224033671}
\definecolor{ccc6_6}{rgb}{0.11176470588235299,0.8197404829072211,0.8867736859200619}
\definecolor{ccc6_7}{rgb}{0.17450980392156867,0.8721195109836108,0.8629289996673897}
\definecolor{ccc7_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc7_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc7_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc7_3}{rgb}{0.0019607843137254832,0.7092813076058535,0.9232891061054894}
\definecolor{ccc7_4}{rgb}{0.0725490196078431,0.7829276104921027,0.9005867023006374}
\definecolor{ccc7_5}{rgb}{0.06470588235294117,0.7752039761111298,0.9032471993461288}
\definecolor{ccc7_6}{rgb}{0.11176470588235299,0.8197404829072211,0.8867736859200619}
\definecolor{ccc7_7}{rgb}{0.19019607843137254,0.883909710213612,0.8566380778638628}
\definecolor{ccc8_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc8_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc8_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc8_3}{rgb}{0.0490196078431373,0.7594049166547072,0.9084652718195236}
\definecolor{ccc8_4}{rgb}{0.11176470588235299,0.8197404829072211,0.8867736859200619}
\definecolor{ccc8_5}{rgb}{0.11960784313725492,0.8267341748257635,0.883909710213612}
\definecolor{ccc8_6}{rgb}{0.1352941176470588,0.8403440716378927,0.8780812480836979}
\definecolor{ccc8_7}{rgb}{0.21372549019607845,0.9005867023006374,0.8469582108244671}
\definecolor{ccc9_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc9_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc9_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc9_3}{rgb}{0.1352941176470588,0.8403440716378927,0.8780812480836979}
\definecolor{ccc9_4}{rgb}{0.19019607843137254,0.883909710213612,0.8566380778638628}
\definecolor{ccc9_5}{rgb}{0.19019607843137254,0.883909710213612,0.8566380778638628}
\definecolor{ccc9_6}{rgb}{0.2529411764705882,0.9256376597815562,0.8301840308155507}
\definecolor{ccc9_7}{rgb}{0.27647058823529413,0.9389883606150565,0.8197404829072211}
\definecolor{ccc10_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc10_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc10_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc10_3}{rgb}{0.19803921568627447,0.8896040127307095,0.853443798888316}
\definecolor{ccc10_4}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc10_5}{rgb}{0.27647058823529413,0.9389883606150565,0.8197404829072211}
\definecolor{ccc10_6}{rgb}{0.36274509803921573,0.9768483177596007,0.7790805745256704}
\definecolor{ccc10_7}{rgb}{0.41764705882352937,0.9916446955107427,0.7513318895568734}
\definecolor{ccc11_0}{rgb}{0.4294117647058824,0.11065268189150083,0.9984636039674339}
\definecolor{ccc11_1}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc11_2}{rgb}{0.27254901960784317,0.34972651120626114,0.9840863373026044}
\definecolor{ccc11_3}{rgb}{0.34705882352941175,0.9712810319161138,0.7867449380334833}
\definecolor{ccc11_4}{rgb}{0.3549019607843137,0.9741386021045101,0.7829276104921028}
\definecolor{ccc11_5}{rgb}{0.43333333333333335,0.9945218953682733,0.7431448254773942}
\definecolor{ccc11_6}{rgb}{0.5274509803921568,0.9990704811844932,0.69169843931937}
\definecolor{ccc11_7}{rgb}{0.5117647058823529,0.9998292504580527,0.700543037593291}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$ & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.091(9) & \cellcolor{ccc1_1!20} 0.068(8) & \cellcolor{ccc1_2!20} 0.057(8) & \cellcolor{ccc1_3!20} 0.057(8) & \cellcolor{ccc1_4!20} 0.059(9) & \cellcolor{ccc1_5!20} 0.060(9) & \cellcolor{ccc1_6!20} 0.061(9) & \cellcolor{ccc1_7!20} 0.066(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.049(7) & \cellcolor{ccc2_1!20} 0.065(8) & \cellcolor{ccc2_2!20} 0.108(10) & \cellcolor{ccc2_3!20} 0.113(11) & \cellcolor{ccc2_4!20} 0.126(12) & \cellcolor{ccc2_5!20} 0.130(12) & \cellcolor{ccc2_6!20} 0.137(13) & \cellcolor{ccc2_7!20} 0.156(14)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.048(7) & \cellcolor{ccc3_1!20} 0.062(8) & \cellcolor{ccc3_2!20} 0.084(9) & \cellcolor{ccc3_3!20} 0.115(11) & \cellcolor{ccc3_4!20} 0.130(12) & \cellcolor{ccc3_5!20} 0.129(12) & \cellcolor{ccc3_6!20} 0.146(13) & \cellcolor{ccc3_7!20} 0.154(14)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.048(7) & \cellcolor{ccc4_1!20} 0.063(8) & \cellcolor{ccc4_2!20} 0.078(9) & \cellcolor{ccc4_3!20} 0.116(11) & \cellcolor{ccc4_4!20} 0.129(12) & \cellcolor{ccc4_5!20} 0.129(12) & \cellcolor{ccc4_6!20} 0.144(13) & \cellcolor{ccc4_7!20} 0.152(14)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.048(7) & \cellcolor{ccc5_1!20} 0.061(8) & \cellcolor{ccc5_2!20} 0.076(9) & \cellcolor{ccc5_3!20} 0.118(11) & \cellcolor{ccc5_4!20} 0.130(12) & \cellcolor{ccc5_5!20} 0.132(12) & \cellcolor{ccc5_6!20} 0.147(13) & \cellcolor{ccc5_7!20} 0.154(14)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.048(7) & \cellcolor{ccc6_1!20} 0.061(8) & \cellcolor{ccc6_2!20} 0.076(9) & \cellcolor{ccc6_3!20} 0.121(11) & \cellcolor{ccc6_4!20} 0.132(12) & \cellcolor{ccc6_5!20} 0.134(12) & \cellcolor{ccc6_6!20} 0.143(13) & \cellcolor{ccc6_7!20} 0.155(14)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.048(7) & \cellcolor{ccc7_1!20} 0.061(8) & \cellcolor{ccc7_2!20} 0.076(9) & \cellcolor{ccc7_3!20} 0.124(11) & \cellcolor{ccc7_4!20} 0.136(12) & \cellcolor{ccc7_5!20} 0.135(12) & \cellcolor{ccc7_6!20} 0.144(13) & \cellcolor{ccc7_7!20} 0.158(14)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.048(7) & \cellcolor{ccc8_1!20} 0.061(8) & \cellcolor{ccc8_2!20} 0.076(9) & \cellcolor{ccc8_3!20} 0.132(12) & \cellcolor{ccc8_4!20} 0.143(12) & \cellcolor{ccc8_5!20} 0.145(13) & \cellcolor{ccc8_6!20} 0.148(13) & \cellcolor{ccc8_7!20} 0.162(14)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.048(7) & \cellcolor{ccc9_1!20} 0.061(8) & \cellcolor{ccc9_2!20} 0.076(9) & \cellcolor{ccc9_3!20} 0.148(12) & \cellcolor{ccc9_4!20} 0.158(13) & \cellcolor{ccc9_5!20} 0.157(13) & \cellcolor{ccc9_6!20} 0.168(14) & \cellcolor{ccc9_7!20} 0.173(15)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.048(7) & \cellcolor{ccc10_1!20} 0.061(8) & \cellcolor{ccc10_2!20} 0.076(9) & \cellcolor{ccc10_3!20} 0.159(13) & \cellcolor{ccc10_4!20} 0.182(14) & \cellcolor{ccc10_5!20} 0.173(14) & \cellcolor{ccc10_6!20} 0.187(15) & \cellcolor{ccc10_7!20} 0.197(16)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.048(7) & \cellcolor{ccc11_1!20} 0.061(8) & \cellcolor{ccc11_2!20} 0.076(9) & \cellcolor{ccc11_3!20} 0.185(14) & \cellcolor{ccc11_4!20} 0.186(15) & \cellcolor{ccc11_5!20} 0.200(15) & \cellcolor{ccc11_6!20} 0.217(17) & \cellcolor{ccc11_7!20} 0.214(17)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.6$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m1r2.tex}}
\end{minipage}

==> tables/m1r2_94.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.18627450980392157,0.47309355683601007,0.9697969360350095}
\definecolor{ccc1_1}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc1_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc1_3}{rgb}{0.38235294117647056,0.18374951781657034,0.9957341762950345}
\definecolor{ccc1_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc1_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc1_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc1_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_0}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc2_1}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_3}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_4}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc2_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc2_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc2_7}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc3_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc3_1}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc3_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_3}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc3_5}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc3_6}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc3_7}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc4_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc4_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc4_2}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc4_3}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc4_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc4_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc4_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc4_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc5_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc5_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc5_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_3}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc5_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_5}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc5_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc5_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc6_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc6_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc6_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_3}{rgb}{0.3196078431372549,0.2795825925967438,0.989980213280707}
\definecolor{ccc6_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc6_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc7_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc7_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc7_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc7_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc7_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc8_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc8_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc8_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc8_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc8_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc9_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc9_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc9_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc9_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc9_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc10_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc10_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc10_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc10_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc10_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc11_0}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc11_1}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc11_2}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_3}{rgb}{0.31176470588235294,0.2913897468893246,0.989091608371146}
\definecolor{ccc11_4}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc11_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$  & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.091(9) & \cellcolor{ccc1_1!20} 0.069(8) & \cellcolor{ccc1_2!20} 0.059(8) & \cellcolor{ccc1_3!20} 0.057(8) & \cellcolor{ccc1_4!20} 0.061(9) & \cellcolor{ccc1_5!20} 0.062(9) & \cellcolor{ccc1_6!20} 0.063(9) & \cellcolor{ccc1_7!20} 0.066(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.088(9) & \cellcolor{ccc2_1!20} 0.067(8) & \cellcolor{ccc2_2!20} 0.059(8) & \cellcolor{ccc2_3!20} 0.059(8) & \cellcolor{ccc2_4!20} 0.060(9) & \cellcolor{ccc2_5!20} 0.061(9) & \cellcolor{ccc2_6!20} 0.062(9) & \cellcolor{ccc2_7!20} 0.068(10)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.085(9) & \cellcolor{ccc3_1!20} 0.066(8) & \cellcolor{ccc3_2!20} 0.060(8) & \cellcolor{ccc3_3!20} 0.059(8) & \cellcolor{ccc3_4!20} 0.061(9) & \cellcolor{ccc3_5!20} 0.060(9) & \cellcolor{ccc3_6!20} 0.061(9) & \cellcolor{ccc3_7!20} 0.069(10)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.085(9) & \cellcolor{ccc4_1!20} 0.065(8) & \cellcolor{ccc4_2!20} 0.061(8) & \cellcolor{ccc4_3!20} 0.067(9) & \cellcolor{ccc4_4!20} 0.062(9) & \cellcolor{ccc4_5!20} 0.061(9) & \cellcolor{ccc4_6!20} 0.062(9) & \cellcolor{ccc4_7!20} 0.070(10)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.084(9) & \cellcolor{ccc5_1!20} 0.065(8) & \cellcolor{ccc5_2!20} 0.062(8) & \cellcolor{ccc5_3!20} 0.068(9) & \cellcolor{ccc5_4!20} 0.062(9) & \cellcolor{ccc5_5!20} 0.061(9) & \cellcolor{ccc5_6!20} 0.062(9) & \cellcolor{ccc5_7!20} 0.070(10)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.084(9) & \cellcolor{ccc6_1!20} 0.065(8) & \cellcolor{ccc6_2!20} 0.062(8) & \cellcolor{ccc6_3!20} 0.068(9) & \cellcolor{ccc6_4!20} 0.062(9) & \cellcolor{ccc6_5!20} 0.062(9) & \cellcolor{ccc6_6!20} 0.062(9) & \cellcolor{ccc6_7!20} 0.070(10)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.084(9) & \cellcolor{ccc7_1!20} 0.065(8) & \cellcolor{ccc7_2!20} 0.062(8) & \cellcolor{ccc7_3!20} 0.069(9) & \cellcolor{ccc7_4!20} 0.062(9) & \cellcolor{ccc7_5!20} 0.062(9) & \cellcolor{ccc7_6!20} 0.063(9) & \cellcolor{ccc7_7!20} 0.070(10)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.084(9) & \cellcolor{ccc8_1!20} 0.065(8) & \cellcolor{ccc8_2!20} 0.062(8) & \cellcolor{ccc8_3!20} 0.069(9) & \cellcolor{ccc8_4!20} 0.062(9) & \cellcolor{ccc8_5!20} 0.062(9) & \cellcolor{ccc8_6!20} 0.063(9) & \cellcolor{ccc8_7!20} 0.070(10)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.084(9) & \cellcolor{ccc9_1!20} 0.065(8) & \cellcolor{ccc9_2!20} 0.062(8) & \cellcolor{ccc9_3!20} 0.069(9) & \cellcolor{ccc9_4!20} 0.062(9) & \cellcolor{ccc9_5!20} 0.062(9) & \cellcolor{ccc9_6!20} 0.063(9) & \cellcolor{ccc9_7!20} 0.070(10)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.084(9) & \cellcolor{ccc10_1!20} 0.065(8) & \cellcolor{ccc10_2!20} 0.062(8) & \cellcolor{ccc10_3!20} 0.069(9) & \cellcolor{ccc10_4!20} 0.062(9) & \cellcolor{ccc10_5!20} 0.062(9) & \cellcolor{ccc10_6!20} 0.063(9) & \cellcolor{ccc10_7!20} 0.070(10)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.084(9) & \cellcolor{ccc11_1!20} 0.065(8) & \cellcolor{ccc11_2!20} 0.062(8) & \cellcolor{ccc11_3!20} 0.069(9) & \cellcolor{ccc11_4!20} 0.062(9) & \cellcolor{ccc11_5!20} 0.062(9) & \cellcolor{ccc11_6!20} 0.063(9) & \cellcolor{ccc11_7!20} 0.070(10)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.12$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m1r2.tex}}
\end{minipage}

==> tables/m2r2_266.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc1_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc1_2}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_3}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_4}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc1_5}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_6}{rgb}{0.28823529411764703,0.3265387128400833,0.9862007473534026}
\definecolor{ccc1_7}{rgb}{0.2803921568627451,0.33815827481581706,0.9851622334675065}
\definecolor{ccc2_0}{rgb}{0.1470588235294118,0.5264321628773557,0.961825643172819}
\definecolor{ccc2_1}{rgb}{0.17843137254901964,0.48391142410030147,0.9682760409157589}
\definecolor{ccc2_2}{rgb}{0.10784313725490197,0.5777738314082511,0.9529420004271566}
\definecolor{ccc2_3}{rgb}{0.12352941176470589,0.5574894393428855,0.9566044195004408}
\definecolor{ccc2_4}{rgb}{0.05294117647058827,0.6459280624867872,0.9389883606150565}
\definecolor{ccc2_5}{rgb}{0.009803921568627416,0.7179119230644418,0.9209055179449537}
\definecolor{ccc2_6}{rgb}{0.025490196078431393,0.7348449670469757,0.9160336012803335}
\definecolor{ccc2_7}{rgb}{0.06470588235294117,0.7752039761111298,0.9032471993461288}
\definecolor{ccc3_0}{rgb}{0.10392156862745094,0.8126223709664456,0.8896040127307095}
\definecolor{ccc3_1}{rgb}{0.2058823529411764,0.8951632913550623,0.8502171357296142}
\definecolor{ccc3_2}{rgb}{0.2529411764705882,0.9256376597815562,0.8301840308155507}
\definecolor{ccc3_3}{rgb}{0.2686274509803921,0.9346797673211106,0.8232529481575873}
\definecolor{ccc3_4}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc3_5}{rgb}{0.4019607843137255,0.9881654720812594,0.7594049166547071}
\definecolor{ccc3_6}{rgb}{0.39411764705882346,0.9862007473534026,0.763398282741103}
\definecolor{ccc3_7}{rgb}{0.4647058823529412,0.9984636039674339,0.7264335740162242}
\definecolor{ccc4_0}{rgb}{0.23725490196078436,0.9160336012803335,0.8369891083319778}
\definecolor{ccc4_1}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc4_2}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc4_3}{rgb}{0.5901960784313725,0.989980213280707,0.6552838500134537}
\definecolor{ccc4_4}{rgb}{0.6607843137254901,0.9682760409157589,0.6124202030492502}
\definecolor{ccc4_5}{rgb}{0.7470588235294118,0.9256376597815563,0.5574894393428855}
\definecolor{ccc4_6}{rgb}{0.8176470588235294,0.878081248083698,0.510631193180907}
\definecolor{ccc4_7}{rgb}{0.8725490196078431,0.8336023852211194,0.47309355683601007}
\definecolor{ccc5_0}{rgb}{0.30000000000000004,0.9510565162951535,0.8090169943749475}
\definecolor{ccc5_1}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc5_2}{rgb}{0.7,0.9510565162951536,0.5877852522924731}
\definecolor{ccc5_3}{rgb}{0.7784313725490195,0.9058734224033673,0.5368665976441802}
\definecolor{ccc5_4}{rgb}{0.9352941176470588,0.77520397611113,0.4291206087726091}
\definecolor{ccc5_5}{rgb}{1.0,0.6916984393193701,0.3727019919909141}
\definecolor{ccc5_6}{rgb}{1.0,0.5159178263577514,0.2677330033224681}
\definecolor{ccc5_7}{rgb}{1.0,0.37270199199091436,0.18980109344182594}
\definecolor{ccc6_0}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc6_1}{rgb}{0.6294117647058823,0.9794097676013659,0.631711006253251}
\definecolor{ccc6_2}{rgb}{0.7392156862745098,0.9302293085467404,0.5625927516198231}
\definecolor{ccc6_3}{rgb}{0.9431372549019608,0.7673626814486971,0.4235485126679244}
\definecolor{ccc6_4}{rgb}{1.0,0.6552838500134535,0.3497265112062611}
\definecolor{ccc6_5}{rgb}{1.0,0.5159178263577514,0.2677330033224681}
\definecolor{ccc6_6}{rgb}{1.0,0.38410574917192575,0.1958454670071669}
\definecolor{ccc6_7}{rgb}{1.0,0.21994635783966857,0.11065268189150082}
\definecolor{ccc7_0}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc7_1}{rgb}{0.6372549019607843,0.9768483177596008,0.6269238058941066}
\definecolor{ccc7_2}{rgb}{0.8490196078431373,0.8534437988883159,0.4892929169339235}
\definecolor{ccc7_3}{rgb}{0.9666666666666666,0.7431448254773945,0.4067366430758004}
\definecolor{ccc7_4}{rgb}{1.0,0.6269238058941065,0.3323547994796596}
\definecolor{ccc7_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc7_6}{rgb}{1.0,0.3265387128400838,0.1655538761841302}
\definecolor{ccc7_7}{rgb}{1.0,0.1106526818915011,0.05541147491597008}
\definecolor{ccc8_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc8_1}{rgb}{0.6450980392156862,0.9741386021045102,0.622112816721474}
\definecolor{ccc8_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc8_3}{rgb}{0.9823529411764707,0.7264335740162241,0.3954512068705426}
\definecolor{ccc8_4}{rgb}{1.0,0.5877852522924732,0.30901699437494745}
\definecolor{ccc8_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc8_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc8_7}{rgb}{1.0,0.012319659535238529,0.006159946638138691}
\definecolor{ccc9_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc9_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc9_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc9_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc9_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc9_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc9_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc9_7}{rgb}{1.0,0.0,0.0}
\definecolor{ccc10_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc10_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc10_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc10_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc10_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc10_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc10_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc10_7}{rgb}{1.0,0.0,0.0}
\definecolor{ccc11_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc11_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc11_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc11_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc11_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc11_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc11_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc11_7}{rgb}{1.0,0.0,0.0}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$ & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.088(9) & \cellcolor{ccc1_1!20} 0.070(8) & \cellcolor{ccc1_2!20} 0.064(8) & \cellcolor{ccc1_3!20} 0.067(9) & \cellcolor{ccc1_4!20} 0.065(9) & \cellcolor{ccc1_5!20} 0.064(9) & \cellcolor{ccc1_6!20} 0.074(10) & \cellcolor{ccc1_7!20} 0.075(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.098(9) & \cellcolor{ccc2_1!20} 0.093(9) & \cellcolor{ccc2_2!20} 0.105(10) & \cellcolor{ccc2_3!20} 0.102(10) & \cellcolor{ccc2_4!20} 0.115(11) & \cellcolor{ccc2_5!20} 0.126(12) & \cellcolor{ccc2_6!20} 0.128(12) & \cellcolor{ccc2_7!20} 0.135(13)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.142(11) & \cellcolor{ccc3_1!20} 0.160(12) & \cellcolor{ccc3_2!20} 0.169(13) & \cellcolor{ccc3_3!20} 0.171(13) & \cellcolor{ccc3_4!20} 0.182(14) & \cellcolor{ccc3_5!20} 0.194(15) & \cellcolor{ccc3_6!20} 0.193(15) & \cellcolor{ccc3_7!20} 0.205(16)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.166(12) & \cellcolor{ccc4_1!20} 0.196(13) & \cellcolor{ccc4_2!20} 0.220(15) & \cellcolor{ccc4_3!20} 0.228(16) & \cellcolor{ccc4_4!20} 0.240(17) & \cellcolor{ccc4_5!20} 0.255(18) & \cellcolor{ccc4_6!20} 0.268(19) & \cellcolor{ccc4_7!20} 0.277(20)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.176(12) & \cellcolor{ccc5_1!20} 0.221(14) & \cellcolor{ccc5_2!20} 0.247(16) & \cellcolor{ccc5_3!20} 0.261(17) & \cellcolor{ccc5_4!20} 0.288(19) & \cellcolor{ccc5_5!20} 0.302(20) & \cellcolor{ccc5_6!20} 0.326(22) & \cellcolor{ccc5_7!20} 0.344(24)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.180(12) & \cellcolor{ccc6_1!20} 0.234(15) & \cellcolor{ccc6_2!20} 0.254(16) & \cellcolor{ccc6_3!20} 0.289(19) & \cellcolor{ccc6_4!20} 0.307(20) & \cellcolor{ccc6_5!20} 0.326(22) & \cellcolor{ccc6_6!20} 0.343(24) & \cellcolor{ccc6_7!20} 0.362(25)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.182(12) & \cellcolor{ccc7_1!20} 0.236(15) & \cellcolor{ccc7_2!20} 0.273(17) & \cellcolor{ccc7_3!20} 0.294(19) & \cellcolor{ccc7_4!20} 0.312(20) & \cellcolor{ccc7_5!20} 0.333(22) & \cellcolor{ccc7_6!20} 0.350(24) & \cellcolor{ccc7_7!20} 0.375(26)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.196(13) & \cellcolor{ccc8_1!20} 0.237(15) & \cellcolor{ccc8_2!20} 0.275(17) & \cellcolor{ccc8_3!20} 0.297(19) & \cellcolor{ccc8_4!20} 0.317(21) & \cellcolor{ccc8_5!20} 0.333(23) & \cellcolor{ccc8_6!20} 0.355(24) & \cellcolor{ccc8_7!20} 0.386(27)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.196(13) & \cellcolor{ccc9_1!20} 0.238(15) & \cellcolor{ccc9_2!20} 0.275(17) & \cellcolor{ccc9_3!20} 0.298(19) & \cellcolor{ccc9_4!20} 0.318(21) & \cellcolor{ccc9_5!20} 0.333(23) & \cellcolor{ccc9_6!20} 0.356(24) & \cellcolor{ccc9_7!20} 0.388(27)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.196(13) & \cellcolor{ccc10_1!20} 0.238(15) & \cellcolor{ccc10_2!20} 0.275(17) & \cellcolor{ccc10_3!20} 0.298(19) & \cellcolor{ccc10_4!20} 0.318(21) & \cellcolor{ccc10_5!20} 0.333(23) & \cellcolor{ccc10_6!20} 0.356(24) & \cellcolor{ccc10_7!20} 0.388(27)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.196(13) & \cellcolor{ccc11_1!20} 0.238(15) & \cellcolor{ccc11_2!20} 0.275(17) & \cellcolor{ccc11_3!20} 0.298(19) & \cellcolor{ccc11_4!20} 0.318(21) & \cellcolor{ccc11_5!20} 0.333(23) & \cellcolor{ccc11_6!20} 0.356(24) & \cellcolor{ccc11_7!20} 0.388(27)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.12$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m2r2.tex}}
\end{minipage}

==> tables/m2r2_292.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.20980392156862748,0.44021574083098725,0.9741386021045101}
\definecolor{ccc1_1}{rgb}{0.2647058823529412,0.3612416661871529,0.9829730996839018}
\definecolor{ccc1_2}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_3}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_4}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc1_5}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_7}{rgb}{0.28823529411764703,0.3265387128400833,0.9862007473534026}
\definecolor{ccc2_0}{rgb}{0.15490196078431373,0.5159178263577511,0.9634931442059831}
\definecolor{ccc2_1}{rgb}{0.11568627450980395,0.5676747161445901,0.9547913248866443}
\definecolor{ccc2_2}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc2_3}{rgb}{0.13137254901960782,0.5472195469221112,0.9583812154701222}
\definecolor{ccc2_4}{rgb}{0.0607843137254902,0.6364742361471413,0.9410892525013715}
\definecolor{ccc2_5}{rgb}{0.009803921568627416,0.7179119230644418,0.9209055179449537}
\definecolor{ccc2_6}{rgb}{0.01764705882352935,0.7264335740162241,0.918486985745923}
\definecolor{ccc2_7}{rgb}{0.056862745098039236,0.767362681448697,0.9058734224033671}
\definecolor{ccc3_0}{rgb}{0.10392156862745094,0.8126223709664456,0.8896040127307095}
\definecolor{ccc3_1}{rgb}{0.2058823529411764,0.8951632913550623,0.8502171357296142}
\definecolor{ccc3_2}{rgb}{0.2529411764705882,0.9256376597815562,0.8301840308155507}
\definecolor{ccc3_3}{rgb}{0.2686274509803921,0.9346797673211106,0.8232529481575873}
\definecolor{ccc3_4}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc3_5}{rgb}{0.4019607843137255,0.9881654720812594,0.7594049166547071}
\definecolor{ccc3_6}{rgb}{0.39411764705882346,0.9862007473534026,0.763398282741103}
\definecolor{ccc3_7}{rgb}{0.4647058823529412,0.9984636039674339,0.7264335740162242}
\definecolor{ccc4_0}{rgb}{0.23725490196078436,0.9160336012803335,0.8369891083319778}
\definecolor{ccc4_1}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc4_2}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc4_3}{rgb}{0.5901960784313725,0.989980213280707,0.6552838500134537}
\definecolor{ccc4_4}{rgb}{0.6607843137254901,0.9682760409157589,0.6124202030492502}
\definecolor{ccc4_5}{rgb}{0.7470588235294118,0.9256376597815563,0.5574894393428855}
\definecolor{ccc4_6}{rgb}{0.8176470588235294,0.878081248083698,0.510631193180907}
\definecolor{ccc4_7}{rgb}{0.8725490196078431,0.8336023852211194,0.47309355683601007}
\definecolor{ccc5_0}{rgb}{0.30000000000000004,0.9510565162951535,0.8090169943749475}
\definecolor{ccc5_1}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc5_2}{rgb}{0.7,0.9510565162951536,0.5877852522924731}
\definecolor{ccc5_3}{rgb}{0.7784313725490195,0.9058734224033673,0.5368665976441802}
\definecolor{ccc5_4}{rgb}{0.9352941176470588,0.77520397611113,0.4291206087726091}
\definecolor{ccc5_5}{rgb}{1.0,0.6916984393193701,0.3727019919909141}
\definecolor{ccc5_6}{rgb}{1.0,0.5159178263577514,0.2677330033224681}
\definecolor{ccc5_7}{rgb}{1.0,0.37270199199091436,0.18980109344182594}
\definecolor{ccc6_0}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc6_1}{rgb}{0.6294117647058823,0.9794097676013659,0.631711006253251}
\definecolor{ccc6_2}{rgb}{0.7392156862745098,0.9302293085467404,0.5625927516198231}
\definecolor{ccc6_3}{rgb}{0.9431372549019608,0.7673626814486971,0.4235485126679244}
\definecolor{ccc6_4}{rgb}{1.0,0.6552838500134535,0.3497265112062611}
\definecolor{ccc6_5}{rgb}{1.0,0.5159178263577514,0.2677330033224681}
\definecolor{ccc6_6}{rgb}{1.0,0.38410574917192575,0.1958454670071669}
\definecolor{ccc6_7}{rgb}{1.0,0.21994635783966857,0.11065268189150082}
\definecolor{ccc7_0}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc7_1}{rgb}{0.6372549019607843,0.9768483177596008,0.6269238058941066}
\definecolor{ccc7_2}{rgb}{0.8490196078431373,0.8534437988883159,0.4892929169339235}
\definecolor{ccc7_3}{rgb}{0.9666666666666666,0.7431448254773945,0.4067366430758004}
\definecolor{ccc7_4}{rgb}{1.0,0.6269238058941065,0.3323547994796596}
\definecolor{ccc7_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc7_6}{rgb}{1.0,0.3265387128400838,0.1655538761841302}
\definecolor{ccc7_7}{rgb}{1.0,0.1106526818915011,0.05541147491597008}
\definecolor{ccc8_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc8_1}{rgb}{0.6450980392156862,0.9741386021045102,0.622112816721474}
\definecolor{ccc8_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc8_3}{rgb}{0.9823529411764707,0.7264335740162241,0.3954512068705426}
\definecolor{ccc8_4}{rgb}{1.0,0.5877852522924732,0.30901699437494745}
\definecolor{ccc8_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc8_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc8_7}{rgb}{1.0,0.012319659535238529,0.006159946638138691}
\definecolor{ccc9_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc9_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc9_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc9_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc9_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc9_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc9_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc9_7}{rgb}{1.0,0.0,0.0}
\definecolor{ccc10_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc10_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc10_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc10_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc10_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc10_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc10_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc10_7}{rgb}{1.0,0.0,0.0}
\definecolor{ccc11_0}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc11_1}{rgb}{0.6529411764705881,0.9712810319161139,0.617278221289793}
\definecolor{ccc11_2}{rgb}{0.8568627450980393,0.8469582108244671,0.4839114241003015}
\definecolor{ccc11_3}{rgb}{0.9901960784313726,0.717911923064442,0.3897858732926794}
\definecolor{ccc11_4}{rgb}{1.0,0.5777738314082512,0.3031526741130436}
\definecolor{ccc11_5}{rgb}{1.0,0.4622038835403133,0.2379351950426188}
\definecolor{ccc11_6}{rgb}{1.0,0.279582592596744,0.14120615182309149}
\definecolor{ccc11_7}{rgb}{1.0,0.0,0.0}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$ & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.087(9) & \cellcolor{ccc1_1!20} 0.077(9) & \cellcolor{ccc1_2!20} 0.064(8) & \cellcolor{ccc1_3!20} 0.067(9) & \cellcolor{ccc1_4!20} 0.065(9) & \cellcolor{ccc1_5!20} 0.064(9) & \cellcolor{ccc1_6!20} 0.064(9) & \cellcolor{ccc1_7!20} 0.074(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.097(9) & \cellcolor{ccc2_1!20} 0.103(10) & \cellcolor{ccc2_2!20} 0.088(9) & \cellcolor{ccc2_3!20} 0.101(10) & \cellcolor{ccc2_4!20} 0.113(11) & \cellcolor{ccc2_5!20} 0.125(12) & \cellcolor{ccc2_6!20} 0.127(12) & \cellcolor{ccc2_7!20} 0.134(13)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.142(11) & \cellcolor{ccc3_1!20} 0.160(12) & \cellcolor{ccc3_2!20} 0.169(13) & \cellcolor{ccc3_3!20} 0.171(13) & \cellcolor{ccc3_4!20} 0.182(14) & \cellcolor{ccc3_5!20} 0.194(15) & \cellcolor{ccc3_6!20} 0.193(15) & \cellcolor{ccc3_7!20} 0.205(16)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.166(12) & \cellcolor{ccc4_1!20} 0.196(13) & \cellcolor{ccc4_2!20} 0.220(15) & \cellcolor{ccc4_3!20} 0.228(16) & \cellcolor{ccc4_4!20} 0.240(17) & \cellcolor{ccc4_5!20} 0.255(18) & \cellcolor{ccc4_6!20} 0.268(19) & \cellcolor{ccc4_7!20} 0.277(20)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.176(12) & \cellcolor{ccc5_1!20} 0.221(14) & \cellcolor{ccc5_2!20} 0.247(16) & \cellcolor{ccc5_3!20} 0.261(17) & \cellcolor{ccc5_4!20} 0.288(19) & \cellcolor{ccc5_5!20} 0.302(20) & \cellcolor{ccc5_6!20} 0.326(22) & \cellcolor{ccc5_7!20} 0.344(24)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.180(12) & \cellcolor{ccc6_1!20} 0.234(15) & \cellcolor{ccc6_2!20} 0.254(16) & \cellcolor{ccc6_3!20} 0.289(19) & \cellcolor{ccc6_4!20} 0.307(20) & \cellcolor{ccc6_5!20} 0.326(22) & \cellcolor{ccc6_6!20} 0.343(24) & \cellcolor{ccc6_7!20} 0.362(25)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.182(12) & \cellcolor{ccc7_1!20} 0.236(15) & \cellcolor{ccc7_2!20} 0.273(17) & \cellcolor{ccc7_3!20} 0.294(19) & \cellcolor{ccc7_4!20} 0.312(20) & \cellcolor{ccc7_5!20} 0.333(22) & \cellcolor{ccc7_6!20} 0.350(24) & \cellcolor{ccc7_7!20} 0.375(26)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.196(13) & \cellcolor{ccc8_1!20} 0.237(15) & \cellcolor{ccc8_2!20} 0.275(17) & \cellcolor{ccc8_3!20} 0.297(19) & \cellcolor{ccc8_4!20} 0.317(21) & \cellcolor{ccc8_5!20} 0.333(23) & \cellcolor{ccc8_6!20} 0.355(24) & \cellcolor{ccc8_7!20} 0.386(27)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.196(13) & \cellcolor{ccc9_1!20} 0.238(15) & \cellcolor{ccc9_2!20} 0.275(17) & \cellcolor{ccc9_3!20} 0.298(19) & \cellcolor{ccc9_4!20} 0.318(21) & \cellcolor{ccc9_5!20} 0.333(23) & \cellcolor{ccc9_6!20} 0.356(24) & \cellcolor{ccc9_7!20} 0.388(27)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.196(13) & \cellcolor{ccc10_1!20} 0.238(15) & \cellcolor{ccc10_2!20} 0.275(17) & \cellcolor{ccc10_3!20} 0.298(19) & \cellcolor{ccc10_4!20} 0.318(21) & \cellcolor{ccc10_5!20} 0.333(23) & \cellcolor{ccc10_6!20} 0.356(24) & \cellcolor{ccc10_7!20} 0.388(27)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.196(13) & \cellcolor{ccc11_1!20} 0.238(15) & \cellcolor{ccc11_2!20} 0.275(17) & \cellcolor{ccc11_3!20} 0.298(19) & \cellcolor{ccc11_4!20} 0.318(21) & \cellcolor{ccc11_5!20} 0.333(23) & \cellcolor{ccc11_6!20} 0.356(24) & \cellcolor{ccc11_7!20} 0.388(27)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.36$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m2r2.tex}}
\end{minipage}

==> tables/m2r2_318.tex <==
\hspace{-9.8cm}
\begin{minipage}[c]{0.7\textwidth}
\resizebox{2.5\textwidth}{!}{
\definecolor{ccc0_0}{rgb}{0.17058823529411765,0.4946558433997788,0.9667184042691874}
\definecolor{ccc0_1}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc0_2}{rgb}{0.3666666666666667,0.20791169081775931,0.9945218953682733}
\definecolor{ccc0_3}{rgb}{0.39803921568627454,0.1594757912099808,0.9967953249171991}
\definecolor{ccc0_4}{rgb}{0.3588235294117647,0.2199463578396686,0.9938591368952737}
\definecolor{ccc0_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc0_6}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc0_7}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_0}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc1_1}{rgb}{0.2647058823529412,0.3612416661871529,0.9829730996839018}
\definecolor{ccc1_2}{rgb}{0.3431372549019608,0.24391372010837714,0.9924205096719357}
\definecolor{ccc1_3}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc1_4}{rgb}{0.33529411764705885,0.2558427775944356,0.9916446955107427}
\definecolor{ccc1_5}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc1_6}{rgb}{0.3509803921568627,0.23194764145389815,0.9931586661366362}
\definecolor{ccc1_7}{rgb}{0.303921568627451,0.30315267411304353,0.9881654720812594}
\definecolor{ccc2_0}{rgb}{0.49215686274509807,0.012319659535238442,0.9999810273487268}
\definecolor{ccc2_1}{rgb}{0.32745098039215687,0.2677330033224679,0.9908312530915603}
\definecolor{ccc2_2}{rgb}{0.10784313725490197,0.5777738314082511,0.9529420004271566}
\definecolor{ccc2_3}{rgb}{0.009803921568627416,0.7179119230644418,0.9209055179449537}
\definecolor{ccc2_4}{rgb}{0.2058823529411764,0.8951632913550623,0.8502171357296142}
\definecolor{ccc2_5}{rgb}{0.2686274509803921,0.9346797673211106,0.8232529481575873}
\definecolor{ccc2_6}{rgb}{0.39411764705882346,0.9862007473534026,0.763398282741103}
\definecolor{ccc2_7}{rgb}{0.4411764705882353,0.9957341762950345,0.7390089172206591}
\definecolor{ccc3_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc3_1}{rgb}{0.24117647058823533,0.3954512068705425,0.9794097676013659}
\definecolor{ccc3_2}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc3_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc3_4}{rgb}{0.19019607843137254,0.883909710213612,0.8566380778638628}
\definecolor{ccc3_5}{rgb}{0.28431372549019607,0.9431544344712774,0.8161969123562217}
\definecolor{ccc3_6}{rgb}{0.4411764705882353,0.9957341762950345,0.7390089172206591}
\definecolor{ccc3_7}{rgb}{0.5274509803921568,0.9990704811844932,0.69169843931937}
\definecolor{ccc4_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc4_1}{rgb}{0.24117647058823533,0.3954512068705425,0.9794097676013659}
\definecolor{ccc4_2}{rgb}{0.22549019607843135,0.41796034488678346,0.9768483177596007}
\definecolor{ccc4_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc4_4}{rgb}{0.3313725490196078,0.965124085200289,0.7942898895752861}
\definecolor{ccc4_5}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc4_6}{rgb}{0.34705882352941175,0.9712810319161138,0.7867449380334833}
\definecolor{ccc4_7}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc5_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc5_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc5_2}{rgb}{0.07647058823529412,0.6172782212897929,0.9451838281608196}
\definecolor{ccc5_3}{rgb}{0.0725490196078431,0.7829276104921027,0.9005867023006374}
\definecolor{ccc5_4}{rgb}{0.2450980392156863,0.9209055179449536,0.8336023852211195}
\definecolor{ccc5_5}{rgb}{0.4019607843137255,0.9881654720812594,0.7594049166547071}
\definecolor{ccc5_6}{rgb}{0.40980392156862744,0.989980213280707,0.7553827347189938}
\definecolor{ccc5_7}{rgb}{0.5274509803921568,0.9990704811844932,0.69169843931937}
\definecolor{ccc6_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc6_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc6_2}{rgb}{0.025490196078431393,0.7348449670469757,0.9160336012803335}
\definecolor{ccc6_3}{rgb}{0.06470588235294117,0.7752039761111298,0.9032471993461288}
\definecolor{ccc6_4}{rgb}{0.307843137254902,0.9547913248866443,0.8053809193888327}
\definecolor{ccc6_5}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc6_6}{rgb}{0.4490196078431372,0.9967953249171991,0.7348449670469757}
\definecolor{ccc6_7}{rgb}{0.5509803921568628,0.9967953249171991,0.678235117349234}
\definecolor{ccc7_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc7_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc7_2}{rgb}{0.07647058823529412,0.6172782212897929,0.9451838281608196}
\definecolor{ccc7_3}{rgb}{0.09607843137254901,0.8053809193888326,0.8924005832479478}
\definecolor{ccc7_4}{rgb}{0.36274509803921573,0.9768483177596007,0.7790805745256704}
\definecolor{ccc7_5}{rgb}{0.38627450980392153,0.9840863373026044,0.767362681448697}
\definecolor{ccc7_6}{rgb}{0.45686274509803915,0.9977051801738729,0.7306531329586932}
\definecolor{ccc7_7}{rgb}{0.7078431372549019,0.9471773565640402,0.582790598933161}
\definecolor{ccc8_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc8_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc8_2}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc8_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc8_4}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc8_5}{rgb}{0.503921568627451,0.9999810273487268,0.7049255469061472}
\definecolor{ccc8_6}{rgb}{0.45686274509803915,0.9977051801738729,0.7306531329586932}
\definecolor{ccc8_7}{rgb}{0.7392156862745098,0.9302293085467404,0.5625927516198231}
\definecolor{ccc9_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc9_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc9_2}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc9_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc9_4}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc9_5}{rgb}{0.5745098039215686,0.9931586661366362,0.6645401787078581}
\definecolor{ccc9_6}{rgb}{0.4647058823529412,0.9984636039674339,0.7264335740162242}
\definecolor{ccc9_7}{rgb}{0.6686274509803922,0.965124085200289,0.6075389463388169}
\definecolor{ccc10_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc10_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc10_2}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc10_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc10_4}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc10_5}{rgb}{0.5745098039215686,0.9931586661366362,0.6645401787078581}
\definecolor{ccc10_6}{rgb}{0.4647058823529412,0.9984636039674339,0.7264335740162242}
\definecolor{ccc10_7}{rgb}{0.6686274509803922,0.965124085200289,0.6075389463388169}
\definecolor{ccc11_0}{rgb}{0.5,0.0,1.0}
\definecolor{ccc11_1}{rgb}{0.2019607843137255,0.4512440570453228,0.9727282722446048}
\definecolor{ccc11_2}{rgb}{0.033333333333333326,0.7431448254773941,0.9135454576426009}
\definecolor{ccc11_3}{rgb}{0.08823529411764708,0.7980172272802395,0.8951632913550623}
\definecolor{ccc11_4}{rgb}{0.3156862745098039,0.9583812154701222,0.8017142839800667}
\definecolor{ccc11_5}{rgb}{0.5745098039215686,0.9931586661366362,0.6645401787078581}
\definecolor{ccc11_6}{rgb}{0.4647058823529412,0.9984636039674339,0.7264335740162242}
\definecolor{ccc11_7}{rgb}{0.6686274509803922,0.965124085200289,0.6075389463388169}
\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
\hline
$\varepsilon \backslash h$ & 1.25e-01& 6.25e-02& 3.12e-02& 1.56e-02& 7.81e-03& 3.91e-03& 1.95e-03& 9.77e-04\\
\hline\hline
0.0 & \cellcolor{ccc0_0!20} 0.094(9) & \cellcolor{ccc0_1!20} 0.071(8) & \cellcolor{ccc0_2!20} 0.060(8) & \cellcolor{ccc0_3!20} 0.054(8) & \cellcolor{ccc0_4!20} 0.061(9) & \cellcolor{ccc0_5!20} 0.063(9) & \cellcolor{ccc0_6!20} 0.064(9) & \cellcolor{ccc0_7!20} 0.066(10)\\
\hline
0.4 & \cellcolor{ccc1_0!20} 0.088(9) & \cellcolor{ccc1_1!20} 0.077(9) & \cellcolor{ccc1_2!20} 0.064(8) & \cellcolor{ccc1_3!20} 0.066(9) & \cellcolor{ccc1_4!20} 0.065(9) & \cellcolor{ccc1_5!20} 0.063(9) & \cellcolor{ccc1_6!20} 0.063(9) & \cellcolor{ccc1_7!20} 0.071(10)\\
\hline
0.8 & \cellcolor{ccc2_0!20} 0.037(7) & \cellcolor{ccc2_1!20} 0.066(8) & \cellcolor{ccc2_2!20} 0.105(10) & \cellcolor{ccc2_3!20} 0.126(11) & \cellcolor{ccc2_4!20} 0.160(13) & \cellcolor{ccc2_5!20} 0.171(14) & \cellcolor{ccc2_6!20} 0.193(15) & \cellcolor{ccc2_7!20} 0.201(16)\\
\hline
1.2 & \cellcolor{ccc3_0!20} 0.036(7) & \cellcolor{ccc3_1!20} 0.081(9) & \cellcolor{ccc3_2!20} 0.084(9) & \cellcolor{ccc3_3!20} 0.140(12) & \cellcolor{ccc3_4!20} 0.157(13) & \cellcolor{ccc3_5!20} 0.174(14) & \cellcolor{ccc3_6!20} 0.202(16) & \cellcolor{ccc3_7!20} 0.217(17)\\
\hline
1.6 & \cellcolor{ccc4_0!20} 0.036(7) & \cellcolor{ccc4_1!20} 0.082(9) & \cellcolor{ccc4_2!20} 0.084(9) & \cellcolor{ccc4_3!20} 0.140(12) & \cellcolor{ccc4_4!20} 0.182(14) & \cellcolor{ccc4_5!20} 0.180(14) & \cellcolor{ccc4_6!20} 0.185(15) & \cellcolor{ccc4_7!20} 0.221(17)\\
\hline
2.0 & \cellcolor{ccc5_0!20} 0.036(7) & \cellcolor{ccc5_1!20} 0.088(9) & \cellcolor{ccc5_2!20} 0.110(10) & \cellcolor{ccc5_3!20} 0.137(12) & \cellcolor{ccc5_4!20} 0.167(14) & \cellcolor{ccc5_5!20} 0.194(15) & \cellcolor{ccc5_6!20} 0.196(16) & \cellcolor{ccc5_7!20} 0.217(17)\\
\hline
2.4 & \cellcolor{ccc6_0!20} 0.036(7) & \cellcolor{ccc6_1!20} 0.088(9) & \cellcolor{ccc6_2!20} 0.129(11) & \cellcolor{ccc6_3!20} 0.135(12) & \cellcolor{ccc6_4!20} 0.178(14) & \cellcolor{ccc6_5!20} 0.180(14) & \cellcolor{ccc6_6!20} 0.203(16) & \cellcolor{ccc6_7!20} 0.221(17)\\
\hline
2.8 & \cellcolor{ccc7_0!20} 0.035(7) & \cellcolor{ccc7_1!20} 0.088(9) & \cellcolor{ccc7_2!20} 0.110(10) & \cellcolor{ccc7_3!20} 0.141(12) & \cellcolor{ccc7_4!20} 0.188(14) & \cellcolor{ccc7_5!20} 0.192(15) & \cellcolor{ccc7_6!20} 0.204(16) & \cellcolor{ccc7_7!20} 0.248(19)\\
\hline
3.5 & \cellcolor{ccc8_0!20} 0.036(7) & \cellcolor{ccc8_1!20} 0.088(9) & \cellcolor{ccc8_2!20} 0.130(11) & \cellcolor{ccc8_3!20} 0.140(12) & \cellcolor{ccc8_4!20} 0.180(14) & \cellcolor{ccc8_5!20} 0.213(16) & \cellcolor{ccc8_6!20} 0.204(16) & \cellcolor{ccc8_7!20} 0.254(19)\\
\hline
5.0 & \cellcolor{ccc9_0!20} 0.036(7) & \cellcolor{ccc9_1!20} 0.088(9) & \cellcolor{ccc9_2!20} 0.130(11) & \cellcolor{ccc9_3!20} 0.140(12) & \cellcolor{ccc9_4!20} 0.180(14) & \cellcolor{ccc9_5!20} 0.225(16) & \cellcolor{ccc9_6!20} 0.205(16) & \cellcolor{ccc9_7!20} 0.241(19)\\
\hline
7.0 & \cellcolor{ccc10_0!20} 0.036(7) & \cellcolor{ccc10_1!20} 0.088(9) & \cellcolor{ccc10_2!20} 0.130(11) & \cellcolor{ccc10_3!20} 0.140(12) & \cellcolor{ccc10_4!20} 0.180(14) & \cellcolor{ccc10_5!20} 0.225(16) & \cellcolor{ccc10_6!20} 0.205(16) & \cellcolor{ccc10_7!20} 0.241(19)\\
\hline
9.5 & \cellcolor{ccc11_0!20} 0.036(7) & \cellcolor{ccc11_1!20} 0.088(9) & \cellcolor{ccc11_2!20} 0.130(11) & \cellcolor{ccc11_3!20} 0.140(12) & \cellcolor{ccc11_4!20} 0.180(14) & \cellcolor{ccc11_5!20} 0.225(16) & \cellcolor{ccc11_6!20} 0.205(16) & \cellcolor{ccc11_7!20} 0.241(19)\\
\hline
\end{tabular}
}
\end{minipage}
\noindent
\hspace{-2.3cm}
\begin{minipage}[c]{0.3\textwidth}\hspace{0.1cm}$\theta=0.6$\\~\\
\resizebox{0.4\textwidth}{!}{\input{images/mu_pattern_m2r2.tex}}
\end{minipage}
